What Could Possibly Go Wrong: Undesirable Patterns in Collective Development

Software development, often perceived as a technical endeavor, is fundamentally a social activity requiring collaboration among team members. Acknowledging this, the software development community has devised strategies to address possible collaboration-related shortcomings. Various studies have attempted to capture the social dynamics within software engineering. In these studies, the authors developed methods to identify numerous teamwork issues and proposed various approaches to address them. However, certain teamwork issues remain unstudied, necessitating a comprehensive bottom-up exploration from practitioner's perceptions to common patterns. This paper introduces the concept of undesirable patterns in collective development, referring to potential teamwork problems that may escalate if unaddressed. Through 38 in-depth exploratory interviews, we identify and classify 42 patterns, revealing their origins and consequences. Subsequent surveys, 436 and 968 participants each, explore the significance and frequency of the undesirable patterns, and evaluate potential tools and features to manage these patterns. The study contributes a nuanced understanding of undesirable patterns, evaluating their impact and proposing pragmatic tools and features for industrial application. The findings provide a valuable foundation for further in-depth studies and the development of tools to enhance collaborative software engineering practices.

==> redundant.tex <==
\section{background}
\subsection{collective development problems}
\subsubsection{community smells}
A social debt itself is a symptom, and it may have many different underlying causes --- community smells~\cite{tamburri2015social}.
A \textbf{community smell} is a set of sub-optimal organizational structures that lead to the emergence and accumulation of both social and technical debt.
The idea of community smells in social debt is similar to the idea of \textit{code smells} in technical debt, the difference is that the former cannot appear in a project developed by a single person.
Community smells primarily produce negative emotions, conflicts, and tense work dynamics, however, community smells might also manifest themselves in code base.


Finally, a set of studies considered community smells in a broader context of collective work.
Palomba et al.~\cite{palomba2018beyond} consider the interconnection between code smells and community smells to create a model predicting code smell intensity from both technical and community-related aspects.
Catolino et al.~\cite{catolino2021understanding} complement the study of Palomba et al.~\cite{palomba2021predicting} by using statistical approach to probe the relationship between various socio-technical patterns and community smells. 
Finally, Catolino et al.~\cite{catolino2020refactoring} carried out an empirical study focused on gauging the relevance of community smells in practice and explored strategies employed by the practitioners to reduce the smells impact. 


\subsubsection{Community smells according to Caballero-Espinosa et al.}
Caballero-Espinosa et al.~\cite{caballero2022community} conducted a systematic literature review which provides an extensive picture of the \cs that the research community had studied.
Together with this review, they also define the connections between community smells (\cs) and factors for effective teamwork. This includes describing \cs properties, a framework for \cs origins and evolution, and a mapping of theoretical connection between community smells and factors for effective teamwork.
As Caballero-Espinosa et al. suggest using their review as a standard reference for studies on community smells, we briefly describe their ideas below.

\textit{List of community smells.}
In their study, Caballero-Espinosa et al. analyze 25 papers to extract 30 different \cs. 
However, the authors notice that the research community has basically focused on 4 \cs: \textit{Organizational Silo, Black Cloud, Lone Wolf, and Radio Silence/Bottleneck}, which, according to e.g.~\cite{de2020splicing,catolino2021understanding} are among the most problematic and impactful.
The majority of the community smells extracted by authors only appear in one to several articles.


\textit{Community smells properties.}
Caballero-Espinosa et al. identify 11 common properties of all 30 \cs they study (such as harmfulness or unpredictability).
For each smell, they also provide causes and effects as defined in the literature. 
Unfortunately, in some instances the causes and \ or effects are either absent in the literature or are formulated in a way which can be obscure for practitioners (e.g. ``undefined information flow'' as an effect of the \textit{Sharing villainy} \cs).
The authors then code the causes and effects to find eight different types of causes such as poor team composition and 11 different types of effects such as emergence of technical debt.
The coding was heavily influenced by the framework of Salas et al.~\cite{salas2015understanding}, which suggests nine critical factors affecting teamwork success.
Caballero-Espinosa et al. also divide the \cs causes into dependent and independent.
The independent causes occur naturally over time given the work setting, while for the dependent causes it is possible to establish a sequence of events which ultimately leads to a \cs.
Finally, the authors utilize the framework of Salas et al. to build a relationship between the community smells and their impact on some of the teamwork success factors.

\textit{Community smell evolution.}
Caballero-Espinosa et al. adopt a five-stage cancer staging framework to represent the evolution of the \cs.
The \cs stages framework depicts community smells as a chronic disease that begins in individuals then spreads across teams and organizations, so that the more advanced stages are more likely to have tangible impact on the software development.
The \cdps as defined Jabrayilzade et al.~\cite{jabrayilzade2022bus} correspond to the stage three to five, and team members may also perceive stage two \cs as a \cdp.


Later studies on the community smells made greater focus on those smells that can be identified in an automatic or semi-automatic fashion. 
For example, in their work, Tamburri et al.~\cite{tamburri2019exploring} introduced CodeFace4Smells --- an automated approach to identify four community smell types: \textit{Organizational Silo, Black Cloud, Lone Wolf, and Radio Silence.}
As these smells manifest themselves in the socio-technical graph of the project, it is possible to create an automated tool that detects these smells.
\textit{Lone Wolf} smell corresponds to a situation in which defiant teammates carry out their work irrespective or regardless of their peers.
As such, it can be identified by a formal rule that identifies a corresponding pattern in the socio-technical graph. 
Further development of community smells detection have extended the methods from the rule-based detection to the machine learning aided detection.
In particular, Palomba et al.~\cite{palomba2021predicting} and Almarimi et al.~\cite{almarimi2020learning} developed models to predict the existence of community smells.
To predict smells, these models use the community-describing metrics, such as social graph betweenness centrality.

\subsection{Team work problems which are not community smells}

% \textit{Community smell} is a set of sub-optimal organizational structures that lead to the emergence and accumulation of both social and technical debt~\cite{caballero2022community}.
% Therefore, a problem in a collective work that is limited to a small group of people may not be caused by the sub-optimal organizational structures and thus cannot be called community smell.
% A community smell corresponds to one or more problems in collective work, as engineers may be unable to identify the issues in the organizational structure which cause particular problems in collective work.

\textit{Collective development problem} is a problem perceived as a factor that already hampers project development~\cite{jabrayilzade2022bus}. 
This is different from the community smells, which may exist but not manifest in additional costs at a certain point of the project life.
Thus, in the initial phase almost any problem in team work may not qualify to be a collective development problem, as it did not exert enough impact.
However, some of the collective development problems identified by Jabrayilzade et al. are not considered to be community smells by the research community (see e.g. Caballero-Espinoza et al.~\cite{espinosa2021understanding} on the community smell classification).


\subsection{Existing tools and approaches}
Software engineering teams rely on a variety of tools to collaborate and streamline workflows. 
These tools facilitate communication, software development and maintenance, project management, and code integration.

\subsubsection{Team work tools}
All the tools we describe below were created to facilitate teamwork, and as such, they mitigate some of the community smells and contribute to appearance of other \cs.
However, their main selling point does not lie in addressing \cs, and when one considers these tools with the \cs optics, one should think how the usage pattern corresponds to the \cs present in a team.

\textit{Version control systems} (VCS) enable teams to track and manage changes to their codebase effectively. 
In particular, engineers can work on code simultaneously, merge changes, and revert to previous versions when needed. 
Platforms such as GitHub, GitLab, and Bitbucket extend this functionality by augmenting VCS repositories hosting with additional features like code review, issue tracking, and collaborative documentation.
Therefore, the data mined from these platforms can be useful in finding \cs that are related to code.
This data can be then used to create tools and plugins to address the \cs.

\textit{Continuous Integration and Deployment (CI/CD) Tools} automate the process of building, testing, and deploying software. 
Jenkins, TeamCity, and CircleCI are popular choices that integrate with version control systems to automatically trigger build and test processes whenever new code changes are pushed. 
These tools enable teams to catch bugs early, ensure code quality, and deliver updates quickly and reliably.
These tools also generate plenty of data, which can be mined to identify both code smells and community smells.
This data can be used to create extensions to address \cs.
For example, from our interviews we find that some software development teams do not strive to keep all tests working.
In this case, an extension to CI/CD tool that monitors whether the status of the tests changed after the update can help engineers to locate outdated tests or breaking changes.

\textit{Documentation Tools} are crucial for maintaining software quality and enabling knowledge sharing within a team. 
Tools like Confluence, Read the Docs, and GitHub Wiki allow teams to create and maintain documentation in a collaborative manner. 
These tools provide a centralized platform for capturing design decisions, APIs, user guides, and troubleshooting instructions, ensuring that information is easily accessible to all team members.
These knowledge bases can be mined to assess if there are knowledge-related \cs, such as lack of documentation or bus factor problem.

\textit{Collaboration and Communication Tools} like Slack, Microsoft Teams, and Google Suite provide instant messaging, file sharing or editing, and video conferencing capabilities, allowing team members to communicate seamlessly and work together on documents. 
These tools often integrate with project management platforms, facilitating the flow of information between team members.
Mining data from these tools may be problematic due to the privacy limitations and general nature of the data (e.g. from the practical point of view it is hard to mine data from a Google Meet meeting).
However, these tools can be augmented by plugins which improve the engineer user experience and mitigate some of the \cs.
For example, a Slack bot which eases writing daily reports and reading reports written by other team members can mitigate \textit{Lone Wolf} \cs.

\textit{Project Management Tools} offer features such as task assignment, progress tracking, and issue management. 
Tools like Jira, YouTrack, or Asana enable teams to break down projects into manageable tasks, set deadlines, allocate resources, and visualize progress through kanban boards, Gantt charts, or burndown charts. 
These tools enhance transparency and coordination within the team, and allow authomatization of some of the tasks.
For example, change of status in a YouTrack issue can trigger an automatic e-mail to an employee providing them instructions for what they need to do next.
Moreover, as the data from these tools is generally available to all employees and easily mineable, one can use it to analyze interaction patterns in the software company. 
As proper usage of these tools creates a map of all work activities in the company, this data can be utilized to analyze and discover most of the \cs.
These tools can be also augmented with plugins and extensions which, by simplifying user's job and reducing the mental burden, can also decrease the frequency of certain \cs.
For example, one can envision a Jira plugin which analyzes the new ticket and checks whether it has enough information and is clear enough so that the responsible employees can work on it.

\textit{All-in-one software development platforms} integrate most of the features the tools described above provide.
Tools like Space, Mattermost, or Phabricator enable teams to keep their activities in a single app and seamlessly move from e.g. reviewing code to updating issue tracking to chat with the colleagues.
Usage of these tools generates lots of data to mine, which eases discovering, analyzing and mitigating \cs.
For example, Jabrayilzade et al.~\cite{jabrayilzade2022bus} report that their bus factor estimation algorithm, which utilized code review and meetings data from Space provided improvement over the baseline algorithm of Avelino et al.~\cite{avelino2016novel}.

\subsubsection{Community smells tools}
To address \cs, an SE team can either use some of the teamwork tools or employ a tool that is designed specifically to mitigate or discover \cs.
These tools can be broadly divided into two groups:

\textit{General-purpose products} such as Qodana, CodeScene, or SonarQube are enterprise tools which provide insights into the quality, health, and maintainability of software codebases. 
As the goal of these tools is to analyze the codebase and its evolution over time to help teams understand the technical debt, complexity, and potential risks associated with the code, they, by proxy, also address some of the community smells that are related to code.
For example, Social Coding Analysis of CodeScene examines collaboration patterns within the development team, highlighting areas where knowledge sharing and communication could be improved. 
This provides insights into how developers work together and identifies bottlenecks or silos, which correspond to some of the community smells identified by our respondents.

\textit{Community smell-focused tools}, as of now, are absent on the market.
The research community developed several tools to address community smells.
Some of these address a particular community smell such as bus factor~\cite{jabrayilzade2022bus,avelino2016novel}, and the others, such as csDetector~\cite{almarimi2021csdetector} or Kaiaulu~\cite{paradis2021design,van2021relations} detect a set of community smells which were first identified by Tamburri et al.~\cite{tamburri2015social}.
Unfortunately, software engineering community did not adopt any of these tools, as these tools are seen as prototypes~\cite{caballero2022community}.


% The observations above motivate us to pose the following research questions:
% \begin{itemize}
%     \item[\textbf{RQ1}] What \up do IT practitioners face in their work?
%     \item[\textbf{RQ2}] What is the relative significance and frequency of the \up?
%     \item[\textbf{RQ3}] What tools might help practitioners address \up?
% \end{itemize}
% To address our first research question, we interview a group of IT practitioners (see~\Cref{sec:design_interview} for more details) in order to collect opinions from employees with diverse IT occupations.
% In these interviews, we also ask respondents to suggest tools which could be used to address the \up they have faced.
% We pose RQ2 to do a rough triage of the \up identified in the interviews.
% Finally, to address RQ3, we survey IT practitioners to find, which of the tool proposals we identified in the interviews are more likely to help them with the \up.
% As opposed to e.g. frameworks or organizational strategies, adopting a tool incurs less switching costs~\todo{find a proof from some good paper about a tool} and thus is more actionable.

\section{motivation}
Meyer et al.~\cite{meyer2019today} show that only 20\% of a software engineer work activity is related to writing code. 
The majority of their time is occupied by activities with direct or indirect social interactions such as meetings, code reviews, discussions at issue trackers, etc.
However, the recently proposed tools and approaches either do not address the problems in collective development directly, or fail to gain traction in the professional community.
The older ideas created to reduce the collective development risks, such as Agile approach~\cite{agile}, are responsible for the emergence of the \cs~\cite{caballero2022community}.  
The review by Caballero-Espinoza et al.~\cite{caballero2022community} shows that while \cs look innocuous, they sabotage software quality.
Thus it is important to address the \cs and limit their impact on the software development process.

Moreover, the research of the \cs is often focused on four particular smells: \textit{Organizational Silo, Black Cloud, Lone Wolf, and Radio Silence/Bottleneck}~\cite{caballero2022community}. 
These smells were first identified in a paper by Tamburry et al~\cite{tamburri2015social}, where authors sought to identify the impact of various community patterns on the decision-making in a large integration project\footnote{The focus on the large-scale patterns is also present in the naming, as researchers use \textit{community} smells and not e.g. \textit{teamwork} smells}.
Therefore, these \cs may be related to the high-level management decisions and thus be hard to capture by the engineers. 
This hypothesis is bolstered by the finding of Caballero-Espinoza~\cite{espinosa2021understanding}, who showed that the perception of \cs he considered is correlated with the manager experience.
Therefore, it is possible that the undesirable patterns in team work which arise in smaller groups and, in each of their instance, affect less people are relatively understudied.


Some of the problems in team work which are related to e.g. code review are not considered to be \cs and fall outside the socio-technical framework as they are not caused by any socio-technical decision.
Therefore, team work problems, which are not directly related to any single well-defined software development practice and are not caused by any socio-technical decisions, may remain invisible to the research community.



Finally, the impact of different approaches to address \cs depends not only on their efficiency if implemented, but also on the likelihood of their implementation.
While socio-technical decision taken in the whole company may fully address a \cs, it also requires a concerted effort of a significant number of employees, and thus is burdened by the switching costs. 
As a switch in operation may come with time and effort costs, some socio-technical changes may be skipped due to the lack of resources or agreement in a team, even if the change will be positive for the team. 
While these costs may be hard to quantify exactly, \cite{jabrayilzade2022bus} have shown that engineers identify these costs as a reason for not addressing \cdps. 



% \textbf{Tangibility of an undesirable pattern.}
% Jabrayilzade et al~\cite{jabrayilzade2022bus} implicitly suggest classifying undesirable patterns into two groups according to the impact perceived by the team members.
% To refine the classification, we suggest the following definitions:
% \begin{itemize}
%     \item[1.] \textit{Community smell} is an undesirable pattern that have not yet resulted in an additional development cost.
%     \item[2.] \textit{Collective development problem} is an undesirable pattern that is perceived as a factor that hampers project development or impacts the costs of the software development (either directly or indirectly).
% \end{itemize}
% The core difference between these two concepts is in the capability of the team to acknowledge the corresponding risks.
% It is important to distinguish between the tangibility and impact.
% For example, a team may perceive having a team member with rare anger outbursts as a collective development problem, but its impact may be minor.
% On the other hand, a Lone Wolf community smell may go on unnoticed and exacerbate for a long time, until some random event (e.g. a sickness of an intermediary colleague just before the release) will suddenly make this community smell a very impactful collective development problem.

% \textbf{Solvability of an undesirable pattern.} \todo{change the name here}
% We propose classifying the undesirable patterns according to the possibility to create a tool that would at least partially help in alleviating them.
% We believe this distinction is important because using a tool that helps with an undesirable pattern may be an easier way to reduce the risks, as compared to changing the social practices adopted in the team \todo{gotta prove it with citations and arguments}.
% Thus we propose the following classification for the undesirable patterns: \todo{choose better names}
% \begin{itemize}
%     \item[1.] \textbf{Human factor undesirable pattern} is an undesirable pattern of imperfect social interaction that cannot be identified from any kind of available data on the software project development and cannot be ameliorated by any kind of a tool.
%     For example, one can imagine that a CEO of a startup creates a very toxic atmosphere at the online meetings which stifles creativity and does not allow for an honest discussion. 
%     This may be a very impactful collective development problem that can even result in dissolution of a company, however it is possible that it will be never manifested in any mineable data such as chats or code base, and it is hard to envision a tool that will help to address toxic behaviour of a startup CEO.
%     \item[2.] \textbf{Manageable undesirable pattern} is an undesirable pattern, which can be alleviated by using a tool. 
%     It does not necessarily mean that this pattern can be somehow identified from the data on the software project. 
%     For example, one can imagine a team with a poor onboarding process, so that the knowledge database of the team does not contain all the information a newcomer may need.
%     While a proper update of a knowledge database tool may resolve the issue, it is unclear how one can automatically determine whether the knowledge database fully covers all the needs of the new engineers.
%     \item[3.] \textbf{Mineable undesirable pattern} is an undesirable pattern, which can be automatically detected by a tool.
%     This category is not a sub-category of the previous category or mutually exclusive with it.
%     An example of a mineable unmanageable undesirable pattern is an issue of choosing components before planning project architecture.
%     While it is possible to create a tool that will identify the projects which have experienced change of composition due to the inadequate planning of project architecture, it is hard to envision a tool that would enforce the team to spend enough time on planning
%     However, even having a tool that simply identifies the undesirable patterns may be beneficial, as it can help to raise the awareness of the team and motivate it to change the processes if needed.
% \end{itemize}

% \todo{Classify existing community smells according to the taxonomy}

\section{methodology}
To the best of our knowledge, there is no exhaustive study of problems in teamwork.
The concept of community smell seem to be strongly related to the problems in collective development.
However, a review by Caballero-Espinoza et al.~\cite{caballero2022community} misses most of the \cdps mentioned by Jabrayilzade et al~.\cite{jabrayilzade2022bus}.
One of the possible explanations is that some of the problems in teamwork are not caused by any socio-technical decision.
Therefore, these problems fall outside the community smell scope and remain invisible to the research community.

Another observation which motivate our methodology is the problem of adopting approaches to manage a problem in teamwork.
For example, a socio-technical decision taken in the whole company requires concerted effort of a significant number of employees.
The corresponding switching costs may cause the team not to implement the change, even if they consider it to be positive.
These costs may be hard to quantify, but engineers identify lack of resources as one of the reasons for not addressing teamwork problems~\cite{jabrayilzade2022bus}.

\subsubsection{Typology and consequences of the undesirable patterns}
We use the following methodology to study the undesirable patterns properties:
\begin{itemize}
    \item[1.] During the interview, after the respondent describes some teamwork problem, we check whether they gave a detailed description of circumstances and consequences of the problem. 
    If in doubt, we ask them follow-up question about the circumstances and the consequences of this problem.
    \item[2.] Each of the two first authors independently creates a classification of the UP types and consequences. 
    \item[3.] In a series of discussions, authors reconcile their classifications to create a list of UP types and a list of their possible consequences.
    \item[4.] We ask \surveyOne survey respondents to choose UP consequences from a closed list we compile in step 3. 
    We only ask this question if the survey respondent have answered in previous question that they faced this particular UP in practice.
    This question also has an open option, where the respondents could add other consequences we failed to mention, but only about 5\% of the respondents have used it.
\end{itemize}
As a result of this scheme, we create classification of the UP types and consequences.
We also validate the consequences classification and gather data on the prevalence of various consequences, which may allow practitioners to do a rough estimate of the risks related to the presence of UP.

\section{discussion}
In our study, we collect a list of 42 \ups, a majority of which correspond to the already known smells.
This list is probably not exhaustive, as we had a limited number of interview respondents, and while we strived to get the most diverse set of respondents, we e.g. could not find respondents from South America. 
Moreover, we conducted our interviews in 2022, and asked our respondents about the \ups they had faced over the last year. 
While asking our respondents only about the events which took place in 2021 or 2022 is reasonable as people can forget important details of the past events, we nevertheless limited the study to the years in which SE industry worldwide was grappling with the consequences of COVID-19.
It would thus be interesting to do a similar qualitative study in a few years to check if some other \ups have emerged, or if the \ups we describe in this paper evolved.
